SoccerNet-Tracking: Multiple Object Tracking Dataset and Benchmark in Soccer Videos

Tracking objects in soccer videos is extremely important to gather both player and team statistics, whether it is to estimate the total distance run, the ball possession or the team formation. Video processing can help automating the extraction of those information, without the need of any invasive sensor, hence applicable to any team on any stadium. Yet, the availability of datasets to train learnable models and benchmarks to evaluate methods on a common testbed is very limited. In this work, we propose a novel dataset for multiple object tracking composed of 200 sequences of 30s each, representative of challenging soccer scenarios, and a complete 45-minutes half-time for long-term tracking. The dataset is fully annotated with bounding boxes and tracklet IDs, enabling the training of MOT baselines in the soccer domain and a full benchmarking of those methods on our segregated challenge sets. Our analysis shows that multiple player, referee and ball tracking in soccer videos is far from being solved, with several improvement required in case of fast motion or in scenarios of severe occlusion.

==> sections/5_analysis.tex <==
%!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!![WARNING] !!!!!!!!!!!!!!!!!!!!!!!!!!!! MOVED TO SECTION 4
% \section{Analysis}
% \label{sec:Analysis}

% \subsection{Analysis of baseline results}
% We evaluate the above baseline methods on our SoccerNet-Tracking test set, and show the results in Table~\ref{table:results}. In the "Setup" column, "w/GT" indicates that ground truth bounding boxes are provided as detection results, while "w/o GT" indicates the usual setting, i.e. each algorithm uses its own detector. Therefore, in the "w/GT" setup we are able to focus our study only on the association performance, given the same perfect detection results for every algorithm.

% Consistently with  the MOT20 benchmark, we obtain increasingly good performance from DeepSORT to FairMOT to ByteTrack without ground truth detections. Given ground truth bounding boxes, ByteTrack outperforms DeepSORT in tracking but only slightly.
% Also, fine-tuning improves both the detection and tracking performance for FairMOT significantly. Let us note that we did not test FairMOT with ground truth detections since the pipeline does not allow easy injection of external detections like DeepSORT and ByteTrack do.
% For all algorithms, there are two  main sources of noise degrading these performance when using the algorithm's own detector: (1) some of the test videos contain audience outside the soccer field, which may cause false positive detections that are note annotated in our dataset as we only focus on objects on the fields, and (2) the detectors are trained for human only, so the ball is never considered in those experiments.

% We also provide a thorough study of the different benchmarks on a per-class action basis in Table \ref{table:hota_categories}. 
% As can be seen, penalty and goal events have the lowest detection scores without ground truth detections. 
% This is consistent with our intuition, since in both scenarios, players tend to gather around the goal and are more likely to be occluded, making it both harder to detect and track. 
% Corners correspond to much harder cases since even given the ground truth bounding boxes, the tracking score remains low as many players gather within the great rectangle. 
% This calls for both better detectors and also trackers that are more robust to occlusion and have improved re-identification capabilities. 
% Finally, substitution events have the highest scores with and without ground truth detections as  these sequences tend to be more static with players usually standing around or moving slowly. 



% \subsection{Qualitative analysis of results}
% %Add Kitti website DetA-AssA trade-off graph

% % good example SNMOT-188 frames 10-20

% % 19  SNMOT-135  41.000  59.928  28.219  63.919  77.479  29.195  77.488  80.916  42.456   53.560   76.214       40.820  ...   1   366  44.799  40.879  49.551   5127  7415  10347    12542  211      24  SNMOT-135  Direct free-kick.
% % frames 175-187 /Users/zhouxin16/Downloads/track_vis/2022_02_04_23_25_19/000175.jpg

% % 22  SNMOT-138  47.942  63.289  36.398  67.234  77.692  40.041  71.627  80.869  49.466   63.095   76.782       48.445  ...   3   253  55.703  51.954  60.035   6500  6011  10827    12511  126      25  SNMOT-138              Foul
% % 217 - 221

% % 26  SNMOT-142  40.479  57.912  28.379  61.503  77.478  29.608  75.414  80.867  41.774   53.413   76.340       40.775  ...   1   359  45.604  40.903  51.527   4521  6532   8774    11053  175      25  SNMOT-142   Shots on target
% % 172 - 239

% % 29  SNMOT-145  42.099  56.774  31.542  60.186  78.255  33.365  77.508  81.447  43.504   54.040   77.026       41.625  ...   1   304  51.937  45.941  59.734   4403  5181   7371     9584  206      25  SNMOT-145            Corner
% % 

% \iffalse
%           seq    HOTA    DetA    AssA   DetRe   DetPr   AssRe   AssPr    LocA   RHOTA  HOTA(0)  LocA(0)  HOTALocA(0)  ...  ML  Frag     IDR     IDP    IDTP   IDFN  IDFP   Dets  GT_Dets  IDs  GT_IDs       name             class
% 0   SNMOT-116  48.382  61.523  38.216  65.816  77.645  42.817  68.422  81.267  50.142   64.635   76.327       49.334  ...   1   221  60.178  55.593  65.586   6371  5089   9714    11460  128      27  SNMOT-116            Corner
% 1   SNMOT-117  64.390  66.660  62.232  70.237  81.476  65.208  82.562  83.396  66.087   81.458   80.224       65.349  ...   2   100  78.328  72.926  84.594   6688  2483   7906     9171  109      31  SNMOT-117           Offside
% 2   SNMOT-118  66.198  69.748  62.914  74.253  81.101  65.848  83.006  83.438  68.329   83.643   79.815       66.760  ...   3   194  80.589  77.187  84.305   8428  2491   9997    10919  107      25  SNMOT-118  Shots off target
% 3   SNMOT-119  67.925  65.786  70.170  69.875  81.106  73.793  82.848  83.581  69.996   86.773   79.937       69.363  ...   4    85  84.739  78.872  91.549   6738  1805   7360     8543   80      26  SNMOT-119         Clearance
% 4   SNMOT-120  51.617  68.961  38.770  72.958  80.700  40.045  82.488  82.792  53.182   65.266   79.389       51.814  ...   2   220  57.374  54.622  60.418   6388  5307  10573    11695  169      27  SNMOT-120              Foul
% 5   SNMOT-121  61.727  70.503  54.093  74.845  79.335  57.932  77.000  81.870  63.603   80.625   78.192       63.042  ...   0   113  75.345  73.213  77.606   8265  3024  10650    11289  104      23  SNMOT-121       Yellow card
% 6   SNMOT-122  47.867  68.984  33.550  73.190  81.277  35.158  79.103  83.377  49.476   59.544   79.878       47.563  ...   1   253  49.749  47.274  52.498   5507  6142  10490    11649  162      26  SNMOT-122  Direct free-kick
% 7   SNMOT-123  63.961  72.492  56.513  76.057  82.344  59.625  81.018  83.591  65.552   79.820   80.795       64.490  ...   1   165  75.231  72.359  78.340   8966  3425  11445    12391  100      25  SNMOT-123   Shots on target
% 8   SNMOT-124  50.197  62.565  40.466  67.069  77.465  42.260  80.174  81.246  52.087   65.907   76.774       50.599  ...   1   202  58.148  54.247  62.655   5263  4439   8400     9702  152      25  SNMOT-124          Kick-off
% 9   SNMOT-125  51.417  62.143  42.665  65.426  79.918  45.500  73.743  82.180  52.831   65.607   78.539       51.527  ...   1   173  60.675  55.174  67.394   5188  4215   7698     9403  114      26  SNMOT-125            Corner
% 10  SNMOT-126  61.209  71.376  52.536  75.179  82.819  54.318  84.449  84.284  62.822   75.578   81.413       61.530  ...   1   131  66.994  63.904  70.398   6754  3815   9594    10569  146      25  SNMOT-126         Clearance
% 11  SNMOT-127  79.528  79.310  79.779  83.249  86.388  82.479  88.234  87.088  81.461   93.593   85.248       79.786  ...   0    58  92.400  90.722  94.142  13210  1351  14032    14561   46      22  SNMOT-127      Substitution
% 12  SNMOT-128  61.799  67.152  56.918  71.905  77.001  59.928  78.879  80.644  63.948   82.987   76.404       63.405  ...   0   189  79.036  76.421  81.837  10647  3285  13010    13932  105      24  SNMOT-128       Yellow card
% 13  SNMOT-129  57.381  71.600  46.066  75.578  81.119  50.181  73.828  82.990  59.000   72.353   79.935       57.836  ...   0   173  66.217  63.956  68.645   7761  4374  11306    12135  120      25  SNMOT-129   Shots on target
% 14  SNMOT-130  64.209  75.252  54.884  79.183  83.930  56.933  85.452  85.037  65.920   78.874   82.369       64.968  ...   0   118  70.995  68.987  73.123   7770  3493  10626    11263   97      21  SNMOT-130  Shots off target
% 15  SNMOT-131  60.886  75.254  49.339  79.417  83.510  51.367  81.234  84.784  62.587   74.772   81.909       61.245  ...   0   200  65.307  63.707  66.991   8824  5027  13172    13851  103      23  SNMOT-131  Direct free-kick
% 16  SNMOT-132  56.395  66.314  48.048  70.561  79.019  50.516  80.726  81.865  58.218   73.667   78.010       57.468  ...   1   271  66.380  62.827  70.358   7173  4244  10195    11417  167      25  SNMOT-132          Kick-off
% 17  SNMOT-133  54.754  63.270  47.492  67.197  77.129  49.999  77.464  80.449  56.487   72.681   76.321       55.471  ...   1   192  70.682  66.131  75.906   8232  4216  10845    12448  142      29  SNMOT-133       Yellow card
% 18  SNMOT-134  57.015  65.363  49.905  69.483  77.400  52.483  78.118  80.594  58.882   74.967   76.367       57.250  ...   0   159  71.740  68.071  75.827   6189  2903   8162     9092  120      23  SNMOT-134           Offside
% 19  SNMOT-135  41.000  59.928  28.219  63.919  77.479  29.195  77.488  80.916  42.456   53.560   76.214       40.820  ...   1   366  44.799  40.879  49.551   5127  7415  10347    12542  211      24  SNMOT-135  Direct free-kick
% 20  SNMOT-136  52.415  63.468  43.342  67.243  78.104  46.587  74.555  81.084  53.976   68.884   77.206       53.182  ...   2   157  65.020  60.499  70.271   5621  3670   7999     9291  111      25  SNMOT-136   Shots on target
% 21  SNMOT-137  60.568  65.423  56.124  70.566  77.220  59.559  77.791  81.472  62.916   79.405   77.602       61.620  ...   1   168  74.411  71.205  77.920   6412  2593   8229     9005  130      25  SNMOT-137         Clearance
% 22  SNMOT-138  47.942  63.289  36.398  67.234  77.692  40.041  71.627  80.869  49.466   63.095   76.782       48.445  ...   3   253  55.703  51.954  60.035   6500  6011  10827    12511  126      25  SNMOT-138              Foul
% 23  SNMOT-139  50.987  67.050  38.851  71.395  78.330  40.365  78.793  81.309  52.661   66.686   77.225       51.498  ...   1   190  59.868  57.217  62.776   6029  4508   9604    10537  122      21  SNMOT-139  Shots off target
% 24  SNMOT-140  47.624  64.896  35.085  70.054  75.704  36.281  78.871  80.296  49.572   63.128   76.173       48.087  ...   1   237  50.751  48.858  52.798   6501  6805  12313    13306  139      23  SNMOT-140            Corner
% 25  SNMOT-141  51.039  64.958  40.138  69.251  78.397  41.970  79.754  81.733  52.705   66.379   78.087       51.833  ...   1   233  61.731  58.130  65.807   6099  4393   9268    10492  174      24  SNMOT-141              Foul
% 26  SNMOT-142  40.479  57.912  28.379  61.503  77.478  29.608  75.414  80.867  41.774   53.413   76.340       40.775  ...   1   359  45.604  40.903  51.527   4521  6532   8774    11053  175      25  SNMOT-142   Shots on target
% 27  SNMOT-143  50.770  59.916  43.129  63.284  78.043  45.458  78.759  80.995  52.240   66.970   76.808       51.438  ...   1   128  61.990  56.128  69.218   4259  3329   6153     7588   88      24  SNMOT-143           Offside
% 28  SNMOT-144  55.383  65.442  46.949  69.413  79.382  49.913  77.858  82.000  57.080   72.119   78.105       56.329  ...   2   169  65.697  61.572  70.414   6119  3819   8690     9938  128      25  SNMOT-144           Penalty
% 29  SNMOT-145  42.099  56.774  31.542  60.186  78.255  33.365  77.508  81.447  43.504   54.040   77.026       41.625  ...   1   304  51.937  45.941  59.734   4403  5181   7371     9584  206      25  SNMOT-145            Corner
% 30  SNMOT-146  61.232  68.930  54.451  72.973  80.371  56.927  82.392  82.574  63.014   79.058   78.992       62.449  ...   1   137  72.982  69.623  76.681   5189  2264   6767     7453   90      22  SNMOT-146  Shots off target
% 31  SNMOT-147  43.041  49.503  37.797  52.204  77.828  39.073  81.989  81.152  44.354   54.621   76.647       41.865  ...   3   202  55.921  46.716  69.646   2930  3342   4207     6272  171      27  SNMOT-147         Clearance
% 32  SNMOT-148  60.151  66.499  54.468  70.435  79.424  56.907  80.956  81.966  61.921   77.833   78.263       60.915  ...   1   171  74.640  70.416  79.403   7205  3027   9074    10232  122      23  SNMOT-148              Goal
% 33  SNMOT-149  61.564  70.545  53.762  73.906  83.193  55.807  83.921  84.285  63.016   76.349   81.638       62.330  ...   2   124  71.746  67.742  76.253   7058  3361   9256    10419   89      24  SNMOT-149          Kick-off
% 34  SNMOT-150  54.336  61.845  47.823  70.272  74.117  49.458  83.545  83.047  57.969   68.153   79.926       54.472  ...   3   150  67.162  65.420  69.000   7049  3726  10216    10775  109      29  SNMOT-150      Substitution
% 35  SNMOT-187  63.024  72.875  54.533  76.592  81.778  59.032  73.404  83.301  64.595   79.549   80.556       64.082  ...   1    78  73.123  70.804  75.599  10416  4295  13778    14711   89      24  SNMOT-187            Corner
% 36  SNMOT-188  68.383  67.493  69.345  72.187  76.667  73.913  77.589  80.270  70.716   92.827   75.953       70.504  ...   1   114  91.783  89.102  94.632  15918  1947  16821    17865   36      27  SNMOT-188      Substitution
% 37  SNMOT-189  56.701  66.308  48.539  70.708  76.478  50.942  77.535  80.000  58.562   76.898   75.604       58.138  ...   1   188  68.618  66.029  71.418   8463  4354  11850    12817  130      25  SNMOT-189              Foul
% 38  SNMOT-190  56.039  59.058  53.191  71.291  66.590  56.303  76.217  80.103  61.542   75.485   75.999       57.368  ...   1   111  69.926  72.394  67.620   8418  3210  12449    11628  109      24  SNMOT-190  Shots off target
% 39  SNMOT-191  64.788  69.264  60.630  74.338  78.455  63.492  80.688  81.989  67.095   84.212   78.426       66.045  ...   1    87  80.973  78.849  83.215   9633  2584  11576    12217   92      24  SNMOT-191           Offside
% 40  SNMOT-192  53.020  63.654  44.254  69.537  72.838  46.354  75.991  78.694  55.460   73.126   73.648       53.855  ...   1   303  64.369  62.910  65.897   7302  4305  11081    11607  158      26  SNMOT-192       Yellow card
% 41  SNMOT-193  47.115  62.252  35.769  67.943  72.385  38.126  73.228  78.509  49.293   65.404   73.508       48.077  ...   1   271  56.869  55.124  58.729   6799  5535  11577    12334  190      26  SNMOT-193  Direct free-kick
% 42  SNMOT-194  59.092  65.958  52.952  70.166  75.464  56.158  75.194  79.128  60.886   81.955   74.580       61.123  ...   1   152  77.113  74.406  80.024  11277  3879  14092    15156   71      24  SNMOT-194         Clearance
% 43  SNMOT-195  61.466  68.290  55.353  74.365  76.091  58.559  76.821  81.154  64.125   80.484   77.624       62.475  ...   1   160  74.101  73.260  74.960   9855  3597  13147    13452  133      22  SNMOT-195  Shots off target
% 44  SNMOT-196  50.736  57.772  44.589  67.541  68.576  46.813  77.530  80.007  54.859   68.915   75.365       51.938  ...   1   275  64.313  63.828  64.805   7277  4124  11229    11401  166      24  SNMOT-196         Clearance
% 45  SNMOT-197  64.901  65.386  64.438  73.877  73.039  67.993  79.186  80.954  68.941   86.632   76.876       66.599  ...   0   185  82.717  83.191  82.248  11532  2330  14021    13862  101      24  SNMOT-197              Foul
% 46  SNMOT-198  54.629  61.277  48.729  68.780  70.687  52.448  73.451  78.794  57.848   76.398   73.812       56.391  ...   2   303  68.933  68.003  69.888  10008  4709  14320    14717  141      27  SNMOT-198  Direct free-kick
% 47  SNMOT-199  45.298  61.329  33.531  68.784  72.804  36.571  68.652  80.540  48.022   60.791   75.714       46.028  ...   2   390  53.783  52.298  55.355   7236  6600  13072    13836  100      25  SNMOT-199            Corner
% 48  SNMOT-200  58.177  64.787  52.316  71.555  74.491  54.470  80.261  80.969  61.174   76.361   77.175       58.932  ...   1   102  69.424  68.056  70.848   8477  3979  11965    12456   88      20  SNMOT-200   Shots on target
% \fi

% % good sequence
% % 119 371 - 389 371, 377, 383, 389


% \begin{figure*}
%     \centering
%     \includegraphics[width=\textwidth]{Submission/figures/examples-tracking.png}
%     \caption{
%     \textbf{Qualitative tracking results.} We show several tracking sequences produced by the ByteTrack algorithm with ground truth detections provided. Sequence (a) shows a good tracking of the players, even after some players or the referee are partially occluded. Sequence (b) shows an example with fast motion, where tracking becomes difficult for both the ball and players due to the distance of bounding boxes between consecutive frames. Sequence (c) show a challenging free-kick event where many players are clustered together resulting in extreme occlusions and poor tracking results.} 
%     \label{fig:qualitative_tracking}
% \end{figure*}


% We show three different sequences for qualitative tracking results analyses in Figure~\ref{fig:qualitative_tracking}. In sequence (a), we can see that the players are well tracked even after some players or the referee partially occlude each other. Sequence (b) shows an example with fast motion. Tracking becomes hard for both the ball and players due to the distance of bounding boxes between consecutive frames. In these fast motion scenarios, there are even further space for improvement beyond the current ground truth. Ground truth bounding boxes are generated by interpolating manually labeled ground truth bounding boxes on dense key-frames. However, for fast moving frames, even the densely selected key-frames are not dense enough and some interpolations may not be perfect. This defect can be observed in the last two images of sequence (b) and also sequence (c). In sequence (c), during the free-kick event, many players are clustered together resulting in extreme occlusions. Existing methods perform very badly in this case. Our hope is that future methods include more context information and therefore have more re-identification capabilities to resolve hard cases like this.

% Finally, we compare FAIRMOT with and without fine tuning on two images sampled from our test set in Figure~\ref{fig:qualitative_finetune_results}.Regarding the first example, we can see that the pre-trained detector does not distinguish between people in the audience or players on the field. However, we can see that the fine-tuned detector has learned the semantic roles of each actor and only detects the players, but not the audience anymore. The second example shows a harder case including fast moving objects. In this case, the fine-tuned detector learns to detect some of the fast moving players but not all of them. This indicates that further work is needed to improve performances, which is why we organize tracking challenges on our new dataset.


% \begin{figure}
%     \centering
%     \includegraphics[width=\linewidth]{Submission/figures/examples-MOT_-finetune_-_2.png}
%     \caption{
%     \textbf{Qualitative fine-tuned results.} Comparison of Fair-MOT predictions with and without fine-tuning on our dataset in the case where ground-truth bounding boxes are not provided. Example 1 shows that the fine-tuned model does not consider the audience anymore in its predictions, while Example 2 shows that in the case of fast motion, the method still struggles to correctly detect the player.
%     }
%     \label{fig:qualitative_finetune_results}
% \end{figure}


% % Detection SNMOT-119
% % frame 342 blurry images
% % 
% % frame 226 detection of people


==> tables/SoccerNetSeries.tex <==

\begin{table}[]
    \centering
    \resizebox{\linewidth}{!}{% <------ Don't forget this %
    \begin{tabular}{l||c|c}
Dataset                                       & Data      & Task(s) \\ \midrule
SoccerNet~\cite{Giancola2018SoccerNet}        & $500$ Games & Action Spotting\\
SN-v2~\cite{Deliege2021SoccerNetv2} (Actions) & $550$ Games & Action Spotting\\
SN-v2~\cite{Deliege2021SoccerNetv2} (Replays) & $550$ Games & Replay Grounding\\
SN-v2~\cite{Deliege2021SoccerNetv2} (Cameras) & $200$ Games & Camera Shot Segmentation\\
SN-v3~\cite{Cioppa2022SoccerNetv3} (BBoxes)  & $33,986$ Images & Player ReID\\
SN-v3~\cite{Cioppa2022SoccerNetv3} (Lanes)   & $33,986$ Images & Pitch Localization\\ 
\midrule
SN-Tracking (ours)  & 201 Sequences & Multiple Object Tracking \\ 
    \end{tabular}
    }
    \caption{\textbf{SoccerNet Series.} Overview of the papers, data nature and tasks available in SoccerNet. While SoccerNet started by focusing on purely temporal annotations, the newest version release spatial features. Our tracking dataset brings a new type of task and data with spatio-temporal annotations within video sequences.}
    \label{tab:SoccerNetSeries}
\end{table}


==> tables/results.tex <==


\begin{table*}[t]
    \centering
    \resizebox{\linewidth}{!}{% <------ Don't forget this %
    \begin{tabular}{l|c||c|c|c|c||c|c|c|c|c|c@{}} 
        % \toprule
        Algorithm     & Setup &   HOTA    &   DetA    &   AssA    &   MOTA    & IDF1   &MT    &ML   &IDFP   &IDFN   &IDsw   \\         \midrule
        DeepSORT & w/ GT       &   69.552  &   82.628  &   58.668  &  \bf  94.844  & 74.125 &1155  &6   &140566 &149320  &4382 \\     
         FairMOT & w/ GT        &   -  &    -  &    -  &    -  &  - & -  & - & - & - & -  \\  
        % FairMOT & w-GT        &   65.954  &   81.891  &   53.216  &   89.689  & 67.829 &1107  &20 &156767 &194378 &18543  \\        
        ByteTrack & w/ GT      & \bf 71.500      & \bf 84.342  &	\bf 60.718  & 94.572  & 74.285 & 1131  &4    &134007  &151694  &7374  \\ \midrule
        DeepSORT & w/o GT      &   36.663  &   40.022  &   33.759  &   33.913  & 45.147 &635   &100  &372706 &291296 &4464 \\       
        FairMOT & w/o GT       &   43.911  &   46.317  &   41.778  &   50.698  & 54.252 &654   &83 &260401 &257472 &3389  \\         
        ByteTrack & w/o GT     & 47.225    &	44.489  &	50.257  &   31.741  & 53.538 & 978   & 74 &432040  &200141  &2187  \\        \midrule
        FairMOT-ft & w/o GT    &  \bf 57.882  &   \bf 66.565  &  \bf  50.492  &  \bf  83.565  & 69.019 &994   &46 &144571 &190881 &4888   \\          
        % FairMOT-ft & w/ GT     &   58.774  &   80.51   &   43.04   &   85.875  & 58.215 &1084  &1084 &202091 &249773 &30614\\         \midrule
        % \bottomrule
    \end{tabular}
    }
    \caption{\textbf{Leaderboard}. Evaluation of the state-of-the-art tracking methods on our new SoccerNet-Tracking test set with and without ground-truth bounding boxes. DeepSort, FairMOT and ByteTrack increasingly improve the performance. Fine-tuning FAIRMOT increases significantly the performance, leading to the first state-of-the-art on our new dataset.}
    \label{table:results}
\end{table*}

% \begin{table*}[t]
%     \centering
%     %\resizebox{\linewidth}{!}{% <------ Don't forget this %
%     \begin{tabular}{c@{}|c|c|c|c|c|c|c|c|c|c@{}} 
%         \toprule
%         Algorithm/setup     &   HOTA    &   DetA    &   AssA    &   MOTA    & IDF1   &MT    &ML   &IDFP   &IDFN   &IDsw   \\ 
%         \midrule
%         DeepSORT/wo-gt      &   36.663  &   40.022  &   33.759  &   33.913  & 45.147 &635   &100  &372706 &291296 &4464 \\
%         \midrule
%         DeepSORT/w-gt       &   69.552  &   82.628  &   58.668  &   94.844  & 74.125 &1155  &6   &140566 &149320  &4382 \\
%         \midrule
%         %FairMOT/wo-gt     &   34.115  &   26.777  &   43.59   &   -54.86  & 36.434 &847   &78 &903144 &237621 &5856  \\ %enhance
%         FairMOT/wo-gt       &   43.911  &   46.317  &   41.778  &   50.698  & 54.252 &654   &83 &260401 &257472 &3389  \\ %original
%         \midrule
%         %FairMOT/w-gt(old)   &   65.397  &   81.659  &   52.478  &   ??????  & ?????? &????? &???  &?????  &?????  &?????\\ %on old gt
%         %FairMOT/w-gt        &   64.217  &   81.526  &   50.689  &   89.594  & 64.421 &1088  &22 &172378  &214392 &14858  \\ %enhance?
%         FairMOT/w-gt        &   65.954  &   81.891  &   53.216  &   89.689  & 67.829 &1107  &20 &156767 &194378 &18543  \\%original
%         \midrule
%         %FairMOT-ft/wo-gt    &   57.184  &   65.81   &   49.842  &   82.597  & 68.16  &981   &59 &147253  &196552  &4801  \\ %enhance
%         FairMOT-ft/wo-gt    &   57.882  &   66.565  &   50.492  &   83.565  & 69.019 &994   &46 &144571 &190881 &4888   \\  %original
%         \midrule
%         %FairMOT-ft/w-gt     &   59.304  &   80.57   &   43.774  &   87.396  & 57.969 &1075  &22 &202692  &251404  &21173 \\ %enhance
%         FairMOT-ft/w-gt     &   58.774  &   80.51   &   43.04   &   85.875  & 58.215 &1084  &1084 &202091 &249773 &30614\\ %original
%         \midrule
%         ByteTrack/wo-gt     & 46.933    &	44.508  &	49.616  &   31.816  & 53.009 &975   &74 &433962  &204339  &2677  \\
%         \midrule
%         ByteTrack/w-gt      & 71.5      &	84.342  &	60.718  & 94.572  & 74.285 &1131  &4    &134007  &151694  &7374  \\

%         \bottomrule
%     \end{tabular}
%     %}
%     \caption{Evaluation results on SoccerNet-Tracking test set.}
%     \label{table:results}
% \end{table*}


% https://docs.google.com/spreadsheets/d/1b5VzENsSHmFPfTGxky-Wue45rN0pk-QKngpTL7qCxdk/edit#gid=0
\begin{table}[t]
    \centering
    \resizebox{\linewidth}{!}{% <------ Don't forget this %
    \begin{tabular}{l||c||c}
    % \hline
Algorithm & \multicolumn{2}{c}{ByteTrack - HOTA (DetA/AssA)} \\
setup & wo-gt & w-gt \\ 
\midrule
% Metric              & HOTA / DetA / AssA & HOTA / DetA / AssA \\ \hline
Clearance           &   49.6 (48.9 / 54.7) &   71.0 (82.2 / 61.7) \\
Corner              &   41.6 (45.5 / 39.7) &\underline{63.9 (83.8 / 49.6)} \\
Direct free-kick    &   46.2 (55.1 / 39.5) &   66.5 (84.5 / 53.2) \\
Foul                &   50.4 (54.8 / 46.9) &\underline{65.7 (82.6 / 53.3)} \\
Goal                &\underline{40.3 (29.6 / 54.8)} &   70.9 (82.2 / 61.2) \\
Kick-off            &   47.6 (49.8 / 46.3) &   69.3 (84.5 / 57.1) \\
Offside             &   46.3 (42.7 / 53.4) &   71.2 (83.3 / 61.1) \\
Penalty             &\underline{31.0 (20.1 / 47.8)} &   70.4 (84.1 / 58.9) \\
Shots off target    &   49.2 (47.5 / 51.9) &   74.0 (84.8 / 65.1) \\
Shots on target     &   46.6 (51.6 / 43.3) &   67.6 (83.3 / 55.4) \\
Substitution        &\bf64.7 (63.1 / 66.3) &\bf84.2 (90.3 / 79.3) \\
Yellow card         &\bf53.5 (54.9 / 52.8) &\bf74.1 (83.6 / 65.7) \\
    \end{tabular}
    }
    \caption{\textbf{Per action class performance.} Comparison of HOTA (DetA/AssA) for different event categories for ByteTrack with and without ground truth detections. The \underline{hardest events} include goals, penalties and corners since many player are clustered, while the \textbf{easiest events} correspond to substitutions and yellow card as players are mostly static.}
    \label{table:hota_categories}
\end{table}


% % https://docs.google.com/spreadsheets/d/1b5VzENsSHmFPfTGxky-Wue45rN0pk-QKngpTL7qCxdk/edit#gid=0
% \begin{table}[t]
%     \centering
%     \resizebox{\linewidth}{!}{% <------ Don't forget this %
%     \begin{tabular}{l||c|c|c||c|c|c}
%     \hline
%         Algorithm & ByteTrack & ByteTrack & ByteTrack & ByteTrack & ByteTrack & ByteTrack \\
%         setup & wo-gt & wo-gt & wo-gt & w-gt & w-gt & w-gt \\ \hline
%         Metric & HOTA & DetA & AssA & HOTA & DetA & AssA \\ \hline
%         Clearance & 49.55 & 48.944 & 54.686 & 70.959 & 82.164 & 61.741 \\ \hline
%         Corner & 41.605 & 45.491 & 39.696 & 63.9 & 83.837 & 49.556 \\ \hline
%         Direct free-kick & 46.192 & 55.128 & 39.528 & 66.528 & 84.52 & 53.184 \\ \hline
%         Foul & 50.442 & 54.807 & 46.896 & 65.71 & 82.616 & 53.323 \\ \hline
%         Goal & 40.264 & 29.585 & 54.804 & 70.914 & 82.197 & 61.241 \\ \hline
%         Kick-off & 47.567 & 49.802 & 46.357 & 69.306 & 84.524 & 57.091 \\ \hline
%         Offside & 46.278 & 42.743 & 53.416 & 71.19 & 83.254 & 61.061 \\ \hline
%         Penalty & 30.999 & 20.116 & 47.776 & 70.354 & 84.09 & 58.911 \\ \hline
%         Shots off target & 49.226 & 47.519 & 51.86 & 74.004 & 84.796 & 65.026 \\ \hline
%         Shots on target & 46.645 & 51.583 & 43.314 & 67.648 & 83.305 & 55.434 \\ \hline
%         Substitution & 64.702 & 63.125 & 66.349 & 84.276 & 90.333 & 79.306 \\ \hline
%         Yellow card & 53.492 & 54.872 & 52.787 & 74.054 & 83.625 & 65.669 \\ \hline
%     \end{tabular}
%     }
%     \caption{\textbf{Per action class performance.} Comparison of HOTA for different event categories for ByteTrack with and without ground truth detections. The hardest events include goals, penalties and corners since many player are clustered, while the easiest event correspond to substitutions as players are mostly static.}
%     \label{table:hota_categories}
% \end{table}


% % \begin{table}[t]
% %     \centering
% %     %\resizebox{\linewidth}{!}{% <------ Don't forget this %

% %     \begin{tabular}{|l|l|l|}
% %     \hline
% %         Algorithm/setup & ByteTrack/wo-gt & ByteTrack/w-gt \\ \hline
% %         Clearance & -12.456 & 91.604 \\ \hline
% %         Corner & 15.199 & 92.705 \\ \hline
% %         Direct free-kick & 57.749 & 95.458 \\ \hline
% %         Foul & 59.294 & 93.683 \\ \hline
% %         Goal & -46.443 & 93.96 \\ \hline
% %         Kick-off & 24.474 & 95.962 \\ \hline
% %         Offside & -19.666 & 93.611 \\ \hline
% %         Penalty & -157.06 & 94.245 \\ \hline
% %         Shots off target & 28.013 & 95.738 \\ \hline
% %         Shots on target & 47.552 & 94.064 \\ \hline
% %         Substitution & 69.14 & 96.067 \\ \hline
% %         Yellow card & 56.02 & 94.322 \\ \hline
% %     \end{tabular}

% %     %}
% %     \caption{MOTA for different categories}
% %     \label{table:mota_categories}
% % \end{table}
